Rethinking the Uncertainty: A Critical Review and Analysis in the Era of Large Language Models

In recent years, Large Language Models (LLMs) have become fundamental to a broad spectrum of artificial intelligence applications. As the use of LLMs expands, precisely estimating the uncertainty in their predictions has become crucial. Current methods often struggle to accurately identify, measure, and address the true uncertainty, with many focusing primarily on estimating model confidence. This discrepancy is largely due to an incomplete understanding of where, when, and how uncertainties are injected into models. This paper introduces a comprehensive framework specifically designed to identify and understand the types and sources of uncertainty, aligned with the unique characteristics of LLMs. Our framework enhances the understanding of the diverse landscape of uncertainties by systematically categorizing and defining each type, establishing a solid foundation for developing targeted methods that can precisely quantify these uncertainties. We also provide a detailed introduction to key related concepts and examine the limitations of current methods in mission-critical and safety-sensitive applications. The paper concludes with a perspective on future directions aimed at enhancing the reliability and practical adoption of these methods in real-world scenarios.

==> ICLR_2025_Template/Figures/sources_of_uncertainty.tex <==

\tikzstyle{my-box}=[
    rectangle,
    draw=hidden-draw,
    rounded corners,
    text opacity=1,
    minimum height=1.5em,
    minimum width=5em,
    inner sep=2pt,
    align=center,
    fill opacity=.5,
]
\tikzstyle{cause_leaf}=[my-box, minimum height=1.5em,
    fill=harvestgold!20, text=black, align=left,font=\scriptsize,
    inner xsep=2pt,
    inner ysep=4pt,
]
\tikzstyle{detect_leaf}=[my-box, minimum height=1.5em,
    fill=cyan!20, text=black, align=left,font=\scriptsize,
    inner xsep=2pt,
    inner ysep=4pt,
]
\tikzstyle{mitigate_leaf}=[my-box, minimum height=1.5em,
    fill=lightgreen!20, text=black, align=left,font=\scriptsize,
    inner xsep=2pt,
    inner ysep=4pt,
]
\begin{figure*}[tp]
    \centering
    \resizebox{0.95\textwidth}{!}{
        \begin{forest}
            forked edges,
            for tree={
                grow=east,
                reversed=true,
                anchor=base west,
                parent anchor=east,
                child anchor=west,
                base=left,
                font=\small,
                rectangle,
                draw=hidden-draw,
                rounded corners,
                align=left,
                minimum width=4em,
                edge+={darkgray, line width=1pt},
                s sep=3pt,
                inner xsep=2pt,
                inner ysep=3pt,
                ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
            }
            [
                Uncertainty in Large Language Model, ver, color=red!100, fill=magenta!30,
                text=black
                [
                    Operational Uncertainry, color=orange!100, fill=orange!100, text width=9em, text=black
                    [
                        Training, color=harvestgold!100, fill=harvestgold!100,  text width=3em, text=black
                        [
                        Data Uncertainty, color=harvestgold!100, fill=harvestgold!60,  text width=6em, text=black
                            [
                                Semantic Ambiguity, color=harvestgold!100, fill=harvestgold!30,  text width=10em, text=black
                            ]
                            [
                                 Linguistic Variability , color=harvestgold!100, fill=harvestgold!30,  text width=8em, text=black 
                            ]
                            [
                                 Errors, color=harvestgold!100, fill=harvestgold!30,  text width=2em, text=black
                            ]
                            [
                                 Bias, color=harvestgold!100, fill=harvestgold!30,  text width=2em, text=black
                            ]
                            [
                                Reliability and Contamination ,color=harvestgold!100, fill=harvestgold!30,  text width=11em, text=black
                            ]
                            [
                                Insufficient Knowledge ,color=harvestgold!100, fill=harvestgold!30,  text width=17em, text=black
                            ]
                        ]
                        [
                        Model Uncertainty, color=harvestgold!100, fill=harvestgold!60, text width=7em, text=black
                            [
                                Parameter Estimation \& Optimization
                                , color=harvestgold!100, fill=harvestgold!30,  text width=14em, text=black
                            ]
                            [
                                Model Architecture \& Hypothesis Space
                                , color=harvestgold!100, fill=harvestgold!30,  text width=15em, text=black
                            ]
                        ]
                    ]
                    [
                        Instruction-Tuning and Alignment
                        , color=cyan!100, fill=cyan!100, text width=13em, text=black
                        [
                        Data Labeling and Human Annotation, color=cyan!100, fill=cyan!60,  text width=14em, text=black
                        ]
                        [
                        Guidelines and Feedback
                        , color=cyan!100, fill=cyan!60,  text width=9.5em, text=black
                        ]
                    ]
                    [
                        Inference
                        , color=lightgreen!100, fill=lightgreen!100, text width=3em, text=black
                            [
                            Distributional Uncertainty
                            , color=lightgreen!100, fill=lightgreen!60,  text width=10em, text=black
                            [
                                     In-Domain Uncertainty
                                 , color=lightgreen!100, fill=lightgreen!30,  text width=9em, text=black
                                ]
                                [
                                     Out-of-Domain Uncertainty
                                 , color=lightgreen!100, fill=lightgreen!30,  text width=11em, text=black
                                ]
                            ]
                            [
                            User Uncertainty
                            , color=lightgreen!100, fill=lightgreen!60,  text width=7em, text=black
                                [
                                     Input Ambiguity
                                 , color=lightgreen!100, fill=lightgreen!30,  text width=6em, text=black
                                ]
                                [
                                    User Bias
                                 , color=lightgreen!100, fill=lightgreen!30,  text width=4em, text=black
                                    % [
                                    %   Parameter Modifying, color=lightgreen!100, fill=lightgreen!30,  text width7em, text=black
                                    % ]
                                    % [
                                    %  Injecting Contradicting Knowlege
                                    %   , color=lightgreen!100, fill=lightgreen!30,  text width=11.5em, text=black
                                    % ]
                                ]
                            ]
                        [
                        Sampling and Decoding Uncertainty
                        , color=lightgreen!100, fill=lightgreen!60,  text width=14em, text=black
                        ]
                    ]
                    % [
                    %     Memory-Editing
                    %     , color=lightgreen!100, fill=lightgreen!60, text width=6em, text=black
                    %     [
                    %     Parameter Modifying, color=lightgreen!100, fill=lightgreen!30,  text width7em, text=black
                    %     ]
                    %     [
                    %     Injecting Contradicting Knowlege
                    %     , color=lightgreen!100, fill=lightgreen!30,  text width=11.5em, text=black
                    %     ]
                    % ]
                ]
                [
                    Output Uncertainty, color=pink!100, fill=pink!100, text width=7em, text=black
                    [
                        Multiple Knowledge Frame
                        , color=pink!100, fill=pink!60, text width=11em, text=black
                    ]
                    [
                        Incomplete Information
                        , color=pink!100, fill=pink!60, text width=9em, text=black
                    ]
                    [
                        Contradicting Information
                        , color=pink!100, fill=pink!60, text width=10em, text=black
                    ]
                    [
                        Lack of Supporting Evidence
                        , color=pink!100, fill=pink!60, text width=11em, text=black
                    ]
                ]
            ]
        \end{forest}
    }
\caption{Our proposed framework for classification of types of uncertainty in Large Language Models, and their main causes and sources}
\label{fig: framework}
\end{figure*}

==> ICLR_2025_Template/Sections/1.introduction.tex <==

%In recent years, 
Large Language Models (LLMs) have %achieved significant advancements, demonstrating 
recently demonstrated remarkable capabilities in various complex reasoning and question-answering tasks \citep{zhao2023survey, Wang_2024, liang2022holistic}. However, despite their potential, LLMs 
%are not without flaws. LLMs 
still face significant challenges in generating erroneous answers \citep{ji2023survey, li2023halueval, huang2023survey}, which can have serious consequences, particularly in domains where high levels of accuracy and reliability are critical. A key issue undermining trust in LLM outputs 
%, and significantly impeding their application in safety-critical systems, 
is the models' lack of transparency and expressiveness in their decision-making processes \citep{zhou2023navigating, lin2023generating, yin2023large, xiao2018quantifying, H_llermeier_2021}, where comprehensively understanding and estimating the model's uncertainty plays a vital role.
%. 
%To address this, uncertainty estimation has emerged as a vital component in developing transparent, reliable, and explainable artificial intelligence (XAI) systems \citep{Abdar_2021, Amodei2016ConcretePI, hendrycks2021unsolved, collins2023human}. 
For example, in the medical field, a physician diagnosing a critical condition like cancer would not only require a high predictive accuracy from the model but also need to understand the uncertainty associated with the case \citep{gawlikowski2022survey}. %Incorporating uncertainty awareness into LLMs enhances their utility across multiple dimensions. For instance, integrating uncertainty quantification enhances model comparisons \citep{DBLP_journals_corr_abs-2003-07892, jiang-etal-2021-know} and allows LLMs to abstain from predictions when uncertainty is too high, crucial in high-stakes scenarios \citep{DBLP_journals_corr_abs-2003-07892, jiang-etal-2021-know, gawlikowski2021survey}. Additionally, understanding uncertainty can pinpoint improvement areas and guide data acquisition strategies \citep{gleave2022uncertainty}.





While the need for quantifying uncertainty in LLMs is widely recognized, %uncertainty is not well-defined in this context, and 
there still lacks a consensus on the interpretation of uncertainty in this new context~\citep{gawlikowski2022survey, mena2021survey, guo2022surveyuncertaintyreasoningquantification,H_llermeier_2021, malinin2018predictive}, which 
%. These inconsistencies
in turn further complicates its estimation. %of uncertainty
%, comparison of different methods, and interpretation of model outputs. 
Terms such as {\textbf{\textit{uncertainty}}, {\textbf{\textit{confidence}}, and {\textbf{\textit{reliability}} are often used interchangeably, yet they refer to distinct concepts that require careful distinction \citep{gawlikowski2021survey}. For instance, an LLM can exhibit a high-confidence response to an inherently uncertain and unanswerable question. However, this response could be contextually inappropriate or factually incorrect, illustrating that high confidence does not necessarily correspond to low uncertainty \citep{gawlikowski2022surveyuncertaintydeepneural}. Thus, the first challenge that remains in the literature is to
%In this paper, we aim to first 
\textit{explicate the definition of uncertainty in the context of LLMs and explore the nuanced differences between these intertwined concepts}. % to enhance the  understanding and practical approaches to identify, estimate and mitigate uncertainty in LLMs. 

Traditionally, uncertainty in deep neural networks (DNNs) is categorized into two types: \textit{aleatoric}, arising from data randomness such as sensor noise, and \textit{epistemic}, stemming from limitations in model knowledge due to insufficient data or unmodeled complexities~\citep{gawlikowski2022survey, mena2021survey, guo2022surveyuncertaintyreasoningquantification, H_llermeier_2021, malinin2018predictive}. Although these categories are widely used in deep learning, they do not fully address the unique challenges of LLMs, which include processing complex text data, managing extremely large parameters, and dealing with often inaccessible training data. Furthermore, the entire lifecycle of LLMs—from pre-training through inference—introduces unique uncertainties, as does the interaction between users and these models. Understanding these different sources of uncertainty is critical, particularly from the perspective of making LLMs more interpretable and robust. 
%To achieve this understanding, the second critical challenge is to design an \textit{inclusive and fine-grained framework that systematically identifies and analyzes the various sources of uncertainty in LLMs}.
Achieving this understanding, however, is not possible without an \textit{inclusive and fine-grained framework that systematically identifies and analyzes the various sources of uncertainty in LLMs}.
% we further aim to propose an inclusive and fine-grained framework that systematically identifies and categorizes the uncertainties in LLMs.
%Achieving this understanding, however, is not possible without an inclusive and fine-grained framework that systematically identifies and categorizes the uncertainties in LLMs. %Thus, we further aim to design a fine-grained framework %is specifically designed 
%to address these unique aspects of LLMs, enhancing understanding of their complex uncertainties and improving interpretation.
%Our fine-grained framework is specifically designed to address these unique aspects of LLMs, enhancing understanding of their complex uncertainties and improving interpretation.

% Traditionally, uncertainty in deep neural networks (DNNs) has been classified into two main types: aleatoric and epistemic~\citep{gawlikowski2022survey, mena2021survey, guo2022surveyuncertaintyreasoningquantification,H_llermeier_2021, malinin2018predictive}. 
% Aleatoric, or statistical, uncertainty arises from inherent randomness in the data, such as noise in sensor readings,  while epistemic, or systematic, uncertainty stems from limitations in model knowledge or structure due to insufficient data or unmodeled complexities. While these uncertainty categories have been broadly utilized across various domains of deep learning \citep{gawlikowski2022survey}, they fall short of fully addressing the unique challenges posed by the characteristics of LLMs, such as extremely large parameters, processing complex text data, and the often inaccessible nature of their training data. Additionally, the lifecycle of LLMs—including pre-training, fine-tuning, and inference—introduces additional sources of uncertainty, many of which are unique to LLMs. Moreover, the interaction between users and these models introduces new dimensions of uncertainty that have not been adequately explored. Our proposed fine-grained framework is tailored to capture the unique operational and output characteristics of LLMs, providing a more precise understanding of their complex uncertainty and improving model interpretation.

Recently, numerous studies have been proposed, aiming to estimate the uncertainty in LLMs~\citep{manakul2023selfcheckgpt, beigi2024internalinspectori2robustconfidence, azaria-mitchell-2023-internal, kadavath2022language, kuhn2023semantic}, and can be broadly divided into four main categories based on their underlying mechanisms: logit-based~\citep{Lin2022TeachingMT, mielke-etal-2022-reducing, jiang-etal-2021-know, kuhn2023semantic}, self-evaluation~\citep{kadavath2022language,manakul2023selfcheckgpt, lin2024generating}, consistency-based~\citep{portillo-wightman-etal-2023-strength, wang2023selfconsistency}, and internal-based~\citep{beigi2024internalinspectori2robustconfidence}. However, given the unique characteristics and nuanced aspects of uncertainty in LLMs, critical questions arise regarding the effectiveness of each type of method in truly capturing uncertainly or other related aspects in the context of LLMs, and which specific sources of uncertainty are being detected across the various stages of an LLM's lifecycle. Answering these questions is vital for developing more reliable and comprehensive approaches to uncertainty estimation in LLMs.

%limitations of each method. Important inquiries include assessing the accuracy of these methods in estimating uncertainty, identifying which specific sources of uncertainty they detect across various stages of an LLM's lifecycle, and evaluating their transferability across different applications. Additionally, it is crucial to determine whether these methods provide insights that could enhance model performance in real-world scenarios.


To address the aforementioned challenges and questions, we conduct a critical review and analysis of studies related to uncertainty and other related concepts, aiming to present a comprehensive survey covering the full spectrum of uncertainty in LLMs, particularly focusing on the interplay between uncertainty concepts, sources, estimation methods, and text data characteristics, which, to the best of our knowledge, is still lacking in this field. In summary, our contributions in this survey are manifold and pioneering: (1) We have standardized definitions for uncertainty and explore related concepts, enhancing communication across the field (Section \ref{sec: definitions}). (2) We are the first to propose a comprehensive framework that analyzes all sources of uncertainty throughout the lifecycle of LLMs, providing deep insights into their origins and effective management strategies (Section \ref{sec: sources}). (3) We evaluate and compare current methods for estimating and evaluating LLM uncertainty, discussing their strengths and limitations (Section \ref{sec: methods}). (4) Finally, we identify future research directions to enhance uncertainty estimation in LLMs, addressing critical gaps and emerging trends for improved reliability and accuracy in critical applications (Section \ref{sec: discussion}).

% To identify the challenges and limitations that this assumption creates, we conduct a comprehensive review of the literature related to uncertainty and confidence estimation in LLMs. We focused on identifying key challenges and factors that should be considered when designing effective uncertainty estimation methods. By doing so, this paper aims to bridge the gap in understanding the full spectrum of uncertainty in LLMs, especially examining the interplay between uncertainty concepts, sources, estimation methods, and the unique characteristics of LLMs.





% \textcolor{teal}{In addition to identifying the sources of uncertainty in LLMs, we also review existing methods for measuring uncertainty and confidence, and divide them into four categories including logit-based, self-evaluation, internal-based, and consistency-based approaches. This categorization improves our understanding of current approaches to uncertainty in LLMs by systematically differentiating between methods according to their underlying mechanisms and specific applications. 
% For each category of methods, we critically assess their strengths, weaknesses, and applicability to address different sources of uncertainty, and highlight their limitations and challenges in specific contexts. Additionally, the calibration and evaluation of uncertainty estimation methods present significant challenges due to the diversity of metrics involved. This paper further aims to provide a detailed analysis of these methods and evaluate their effectiveness in capturing uncertainty in LLM outputs.}
%Furthermore, evaluating uncertainty estimation methods presents a significant challenge, especially in Natural Language Generation (NLG) tasks. The variety of metrics used for assessing uncertainty adds complexity to this evaluation, as the metrics must be carefully aligned with the uncertainty estimation methods to avoid inconsistencies. Our survey provides an in-depth analysis of these metrics and evaluates their effectiveness in capturing uncertainty in LLM outputs.



% \textcolor{teal}{Despite significant research on uncertainty in LLMs, a comprehensive survey covering the full spectrum of uncertainty in LLMs, particularly focusing on the interplay between uncertainty concepts, sources, estimation methods, and text data characteristics, is lacking. This paper aims to bridge this gap by providing a detailed examination of uncertainty in LLMs. In this paper, we conduct a comprehensive analysis of uncertainty sources throughout the lifecycle of LLMs, examining how text's unique complexities contribute to this uncertainty.  We review and categorize existing methods for measuring uncertainty and confidence, enhancing our understanding by systematically distinguishing between methods based on their mechanisms. For each category of methods, we critically assess and compare their strengths, weaknesses, and applicability to address different sources of uncertainty, and highlight their limitations and challenges. Additionally, the calibration and evaluation of uncertainty estimation methods present significant challenges due to the diversity of metrics involved. Our paper provides a detailed analysis of these methods and evaluates their effectiveness in capturing uncertainty in LLM outputs.}\lifu{need to rewrite this paragraph to better connect it with the previous two challenges, highlight the literature review we have done, motivate why we also review the literature of uncertainty estimation or what questions/challenges we want to address with that}
 




==> ICLR_2025_Template/Sections/2.definitions.tex <==
\section{Definition of Uncertainty and Related Concepts}
\label{sec: definitions}

%In this section, we first 
This section begins by offering a comprehensive definition of \textit{\textbf{uncertainty}} and its associated concepts—\textbf{\textit{confidence and reliability}}—within the context of large language models. As illustrated in Figure \ref{fig: overview}, although these concepts are interrelated, they pertain to distinct aspects of model performance that necessitate careful differentiation. We specifically emphasize the differences between \textit{uncertainty} and \textit{confidence}, terms that are often used interchangeably in the literature.

\begin{figure*}[!h]
    \centering
    \includegraphics[width=0.9\linewidth]{ICLR_2025_Template/Figures/concept.pdf}
    \caption{Visualization of the Distinct Aspects of Uncertainty, Confidence, and Reliability in Large Language Models}
    \label{fig: overview}
\end{figure*}

\textit{\textbf{Uncertainty}} fundamentally refers to the extent to which a model ``\textbf{knows}'' or ``\textbf{does} \textbf{not} \textbf{know}'' about a given input, based on the training it has received \citep{malinin2018predictive, der2009aleatory, H_llermeier_2021, gawlikowski2022survey, kendall2017uncertainties}. Often, this arises from inadequate or conflicting training data \citep{guo2022surveyuncertaintyreasoningquantification, H_llermeier_2021, mena2021survey}, inappropriate model selection \citep{gawlikowski2022survey,mena2021survey, battaglia2018relationalinductivebiasesdeep}, or factors like noise and inherent data ambiguity \citep{kendall2017uncertainties, mena2021survey, guo2022surveyuncertaintyreasoningquantification}. These factors collectively delineate a model’s understanding—or misunderstanding—of its operational environment, influencing the reliability of its outputs. %of its performance and the cautiousness with which its outputs should be used.

\textit{\textbf{Confidence}}, often expressed as a predicted probability score, quantifies the likelihood that a model’s prediction is correct. Derived from the softmax output applied to logits, this score assigns each class a probability between 0 and 1, with the highest probability indicating the model’s chosen prediction \citep{he2024surveyuncertaintyquantificationmethods, guo2017calibration, nandy2021maximizingrepresentationgapindomain}. However, confidence scores can be misleading; they may exhibit \textbf{overconfidence}, where the score is high despite inaccurate predictions, or\textbf{ underconfidence}, where scores are low even when predictions are correct \citep{lakshminarayanan2017simple, wang2023calibration, chen2022close,guo2017calibration}. 

%The challenges of overconfidence and underconfidence have heightened the need for model \textit{\textbf{reliability}}. 
\textit{\textbf{Reliability}}. Merely estimating confidence scores is insufficient for safe decision-making. It's vital to align confidence scores with the actual probabilities of correct predictions, a process known as calibration \citep{guo2017calibration, wang2023calibration}. Re-calibration techniques have been developed to enhance this alignment, ensuring that confidence estimates are accurately calibrated and reliable for practical applications \citep{guo2017calibration, wang2023calibration, nixon2019measuring, mukhoti2020calibrating}.

\textbf{Does High Confidence Score Always Mean Low Uncertainty?}
Confidence scores are often interpreted as indicators of uncertainty, leading to significant challenges. DNNs frequently assign high confidence to inputs far removed from their training data, resulting in misleading confidence levels for incorrect classifications \citep{hein2019relunetworksyieldhighconfidence}. For instance, a network trained on images of cats and dogs might confidently, but incorrectly, classify a bird as one of these categories \citep{gawlikowski2022survey, malinin2019reverse}. Therefore, high confidence does not necessarily indicate low uncertainty, making such an assumption problematic. LLMs also exhibit high confidence even when uncertainty is substantial. For example, models might confidently answer ambiguous or unanswerable questions like ``\textit{How many planets are in the universe?}'' (\textbf{known unknowns}), ``\textit{What will be the top performing stock in 10 years?}'' (\textbf{future unknowns}), ``\textit{What is consciousness and how does it work?}'' (\textbf{controversial unknowns}), or ``\textit{What is the exact weight of a watermelon?}'' (\textbf{ambiguous questions}), despite the inherent uncertainty of such questions. Similarly, models may express high certainty in speculative or hypothetical scenarios, like ``\textit{What would happen if the US had lost the Independence War?}'', even when no definitive answer exists. These examples highlight that a high confidence score which derived through various computational methods, often imply as zero uncertainty, does not necessarily indicate the correctness of an answer.  It is crucial, therefore, to approach high confidence scores with caution and to develop methods to measure the true uncertainty. 



% It is crucial, therefore, to approach high confidence scores with caution and develop methods to accurately measure true uncertainty. Distinguishing between confidence and uncertainty is key for a deeper understanding, as a thorough grasp of uncertainty and its sources requires a clear foundational framework. In the next section, we propose a comprehensive framework specifically designed to address the unique operational and output characteristics of LLMs.





==> ICLR_2025_Template/Sections/3.types.tex <==
% \section{A Comprehensive Framework for Understanding Uncertainty in Large Language Models}
% \label{sec: types}

\section{Sources of Uncertainty in Large Language Models}
\label{sec: sources}
%To effectively develop methods for identifying and estimating uncertainties in LLMs, a thorough understanding of the sources and dynamics of uncertainties throughout the model's life-cycle is crucial. This includes recognizing text as a unique data type with inherent distinctive features and acknowledging the role of LLMs as knowledge providers for downstream reasoning and decision-making tasks. In this section, we discuss why traditional uncertainty categorizations fall short for LLMs and introduce a structured framework to identify their various sources of uncertainty effectively.

\subsection{A Comprehensive Framework for Understanding Uncertainty in LLMs}


There are three traditional categories of uncertainty commonly used in deep learning, including  %\textit{\textbf{model (or epistemic) uncertainty}}, \textit{\textbf{data (or aleoteric) uncertainty}}, and \textit{\textbf{distributional uncertainty}}. 
(1) \textbf{Model (epistemic) Uncertainty}, which pertains to uncertainties in estimating model parameters, reflecting model fit and its limitations in generalizing to unseen data \citep{der2009aleatory, lahlou2023deup, H_llermeier_2021, malinin2018predictive}; (2) \textbf{Data (or aleoteric) Uncertainty} that stems from complexities within the data itself, such as class overlap and various types of noise \citep{der2009aleatory, rahaman2020uncertainty, wang2019aleatoric, malinin2018predictive}; and (3) \textbf{Distributional Uncertainty}, which often dues to dataset shift and occurs when training and testing data distributions differ, leading to potential generalization issues during real-world applications where the model faces data markedly different from what it was trained on \citep{malinin2018predictive, nandy2021maximizingrepresentationgapindomain, gawlikowski2022survey, chen2019variationaldirichletframeworkoutofdistribution, mena2020uncertainty}.
% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=0.9\linewidth]{ICLR 2025 Template/Figures/framework.png}
%     \caption{Caption}
%     \label{fig: framework}
% \end{figure}
% \begin{wrapfigure}{l}{\textwidth} 
%     \centering
% \includegraphics[width=\textwidth]{ICLR 2025 Template/Figures/framework.png}
%     \caption{Caption}
%     \label{fig: framework}
% \end{wrapfigure}


% There are three traditional categories of uncertainty commonly used in deep learning, including \textit{\textbf{model uncertainty}}, \textit{\textbf{data uncertainty}}, and \textit{\textbf{distributional uncertainty}}. Model uncertainty refers to uncertainty in the estimation of model parameters based on the training data. It reflects how well the model fits the data and highlights its limitations in generalizing to unseen data \citep{der2009aleatory, lahlou2023deup, H_llermeier_2021, malinin2018predictive}. Data uncertainty arises from the inherent complexity of the data itself, such as class overlap, label noise, or the presence of both homoscedastic and heteroscedastic noise \citep{der2009aleatory, rahaman2020uncertainty, wang2019aleatoric,malinin2018predictive}. Distributional uncertainty occurs when there is a mismatch between training and testing data distributions, often known as \textit{dataset shift} \citep{malinin2018predictive, nandy2021maximizingrepresentationgapindomain, gawlikowski2022survey, chen2019variationaldirichletframeworkoutofdistribution, mena2020uncertainty}. This uncertainty is particularly prevalent in real-world scenarios where the model encounters data significantly different from the training data in prediction time. Such changes may introduce uncertainty due to a potential lack of
% generalization of the model, as it requires that the model predicts data points that are different
% from those seen during training. 

\begin{wrapfigure}{rh}[0pt]{0.6\textwidth}
  \centering
  \vspace{-1.8cm}
  \includegraphics[width=0.6\textwidth]{ICLR_2025_Template/Figures/framework2.png}
  \caption{A comprehensive framework to categorize the sources of uncertainty through LLM's life-cycle.}
  \label{fig: framework}
  \vspace{-0.5cm} % !! uncomment this line if there are empty lines at the beginning of the next page  
\end{wrapfigure}
These traditional uncertainty categories, though prevalent in deep learning, fail to fully address the unique challenges of LLMs. LLMs are characterized by extensive parameters, complex text data processing, and often limited access to training data, introducing specific uncertainties in their outputs. Moreover, interactions with users in dynamic environments and human biases in data annotation or model alignment complicate the uncertainty landscape. Unlike general deep learning models that primarily predict numerical outputs or classes, LLMs generate knowledge-based outputs which may include inconsistent or outdated information \citep{lin2024navigatingdualfacetscomprehensive}. These features cannot be adequately addressed by simply categorizing uncertainty into three traditional types. These distinctive aspects necessitate a comprehensive framework to better understand the diverse sources of uncertainty in LLMs. 


To address these challenges, we introduce a new framework to categorize uncertainty in LLMs, as illustrated in Figure \ref{fig: framework}. This framework distinguishes between \textbf{\textit{operational} uncertainty}, which pertains to model and data processing, and \textbf{\textit{output uncertainty}}, focusing on the quality of the generated content. Specifically:
%providing a clearer approach to managing the specific uncertainties faced by LLMs. Operational uncertainty pertains to model and data processing, while output uncertainty focuses on the quality of the generated content.

\textit{\textbf{Operational uncertainty}} in LLMs arise from pre-training to inference, encompassing data acquisition, model and architecture design, training and optimization processes, alignment, and inference activities. These uncertainties stem from how LLMs are trained on extensive datasets, process inputs, and generate text. In essence, operational uncertainties arise when the model is unable to capture the full complexity of the data it has been trained on, or when the input data itself introduces ambiguities or noise. 

\textit{\textbf{Output uncertainty}} in LLMs stems from challenges in analyzing and interpreting the generated text, relating to the quality and reliability of information used for decision-making. For example, in medical scenarios, where an LLM is tasked with providing diagnostic suggestions based on patient symptoms, the model may generate multiple possible diagnoses. However, if these suggestions lack justification or supporting evidence, or contain contradictory information, significant uncertainty arises for the physician who must determine the credibility of these diagnoses. The physician may face substantial challenges in deciding which diagnosis to investigate further, highlighting the critical need for LLMs to provide well-supported, consistent, and reliable outputs to ensure their practical utility in decision-making processes.

By distinguishing between operational and output uncertainties, our framework offers several benefits: first, a fine-grained approach that captures the unique features of LLMs, providing a precise reflection of uncertainty for better modeling and understanding. Second, it establishes a foundation for identifying uncertainty sources, essential for developing targeted methods to accurately quantify them. Third, it offers stakeholder-specific insights, helping developers, users, and administrators address uncertainties relevant to their roles, enhancing model robustness, user interaction, and governance. Lastly, by aggregating beliefs and evaluating output evidence, the framework builds trust in LLM outputs, particularly in critical fields like medical diagnosis or legal reasoning.

% By distinguishing between operational and output uncertainties, our framework enhances the understanding and management of uncertainties inherent in LLMs. This framework offers several benefits: First, it provides a fine-grained approach tailored to capture all unique features of LLMs, offering a more precise reflection of the multidimensional nature of uncertainty, which facilitates better modeling and a deeper understanding. Secondly, it establishes an inclusive foundation for pinpointing the sources of uncertainty, crucial for developing targeted methods to accurately identify and quantify these uncertainties. Third, it delivers stakeholder-specific insights, enabling developers, users, and administrators to understand and address uncertainties pertinent to their roles, thereby enhancing model robustness, user interaction, and governance. Finally, our framework enhances trust in LLM outputs by aggregating beliefs, crucial in fields like medical diagnosis or legal reasoning. By evaluating operational uncertainties and output evidence, we provide a clearer picture of LLM reliability, helping to aggregate evidence and identify inconsistencies or gaps that might affect decision-making processes.



% \begin{figure}[ht]
%   \centering
%   \includegraphics[width=0.7\textwidth]{ICLR 2025 Template/Figures/framework.png}
%   \caption{Our Proposed Framework}
%   \label{fig:exampleImage}
% \end{figure}


% \textbf{Operational Uncertainties:} Operational uncertainties refer to those that emerge from the operational mechanisms of LLMs, from pre-training to inference. These uncertainties include data acquisition process, model and architecture design choices, training and optimization processes, alignment and feedback mechanisms, and inference time. These uncertainties are tied to the way that LLMs are trained on massive corpora, process input data, and generate text. For instance, inaccuracies, biases, or missing data in the pre-training phase can introduce uncertainties that propagate through the model, affecting its output. Similarly, decisions related to model architecture—such as parameter choices, optimization techniques, and hyperparameter tuning—can contribute to operational uncertainties. 
% In essence, operational uncertainties arise when the model is unable to capture the full complexity of the data it has been trained on, or when the input data itself introduces ambiguities or noise. 

% \textbf{Output Uncertainties:} 
% Output uncertainty arises from the challenges in analyzing and interpreting the text generated by LLMs. 
% It is not tied to the model's operational processes but to the quality of the information generated by LLMs, e.g., the reliability, coherence, and completeness of the LLM outputs for downstream decision-making. 
% For example, in medical scenarios, where an LLM is tasked with providing diagnostic suggestions based on patient symptoms, the model may generate multiple possible conditions and diagnoses. However, if these suggestions lack justification or supporting evidence from medical literature, or contain contradictory information, significant uncertainty arises for the physician who must determine the credibility of these diagnoses. The physician may face substantial challenges in deciding which diagnosis to investigate further, highlighting the critical need for LLMs to provide well-supported, consistent, and reliable outputs to ensure their practical utility in decision-making processes.








    










==> ICLR_2025_Template/Sections/4.sources.tex <==
% \section{Sources of Uncertainty in Large Language Models}
% \label{sec: sources}

% \subsection{Operational Uncertainty in Pre-Training and Training Stage of Large Language Model}
\subsection{Operational Uncertainty in LLMs}

\subsubsection{Operational Uncertainty in Pre-Training and Training Stage of LLMs}
\paragraph{\uline{Data Uncertainty}}
This phase involves collecting and organizing the pre-training corpus, which is critical as the quality, diversity, and representativeness of the data directly affect the model's understanding and ability to generalize. The sources of uncertainty at this stage include:

\textbf{\textit{(1) Semantic Ambiguity:}} Textual data inherently contain semantic complexities, leading to significant uncertainties in training and inference processes for language models. For example, the word 'bank' can mean a financial institution or a river's edge, and 'lead' can refer to the act of leading or the metal, depending on the context \citep{10.1007/s00354-022-00162-6, ott2018analyzinguncertaintyneuralmachine, dreyer2012hyter, blodgett-etal-2020-language}. These semantic ambiguities pose challenges in maintaining meaning across different contexts and highlight the difficulty of achieving consistent semantic understanding. Such ambiguities are a primary source of uncertainty, complicating the model's understanding \citep{10.1007/s00354-022-00162-6, Piantadosi2011TheCF}.

\textbf{\textit{(2) Linguistic Variability:}} Textual environments are dynamic and subject to contextual and cultural shifts that significantly alter data interpretation and relevance \citep{kutuzov-etal-2018-diachronic, levy-2008-noisy}. For example, word meanings and usages evolve, new slang emerges, and topics range from casual conversations to specialized discussions, each with distinct linguistic nuances \citep{levy-2008-noisy, liu-etal-2018-neural-relation, kutuzov-etal-2018-diachronic}. This variability requires language models to continually interpret context to determine meaning, greatly increasing the uncertainty in their knowledge and response. 

\textbf{\textit{(3) Errors:}} The data collection process can introduce errors like typographical mistakes, incorrect tagging, or grammatical errors. These inconsistencies can significantly mislead the learning process, impairing the LLM’s ability to model and generate text accurately \citep{wang2024resiliencelargelanguagemodels, liu-etal-2018-neural-relation}. 

\textbf{\textit{(4) Insufficient Coverage:}} This refers to situations where incomplete coverage in the training dataset leads to uncertainty. Mitigating this requires acquiring more extensive and diverse data that encompasses various viewpoints \citep{gawlikowski2022survey}.

\textbf{\textit{(5) Reliability and Contamination of Data:}} Training data for LLMs often contains inaccuracies or outdated content \citep{lin2024navigatingdualfacetscomprehensive}, which can lead these models to perpetuate and amplify such errors \citep{lin2024navigatingdualfacetscomprehensive}. Misrepresented facts and contaminated data—incorrect or misleading information included in the training set—introduce significant uncertainty and hinder the models' reliability as decision-making tools \citep{jiang2024investigatingdatacontaminationpretraining}. 

\textbf{\textit{(6) Human Biases:}} In training data related to gender, race, socio-economic status, age, or disability are primary sources of uncertainty in LLM predictions \citep{bender-friedman-2018-data}. These biases skew the model's understanding and responses, resulting in outputs that may not be universally valid or appropriate, thus increasing uncertainty about the model's performance and reliability in diverse real-world scenarios \citep{kirk2021biasoutoftheboxempiricalanalysis}.

\paragraph{\uline{Model Uncertainty}}
This type primarily arises from the model’s fit to the data, highlighting its ability to generalize from the training data to unseen data \citep{malinin2018predictive}. The design of the architecture and the training process of an LLM are crucial in shaping its capabilities and effectiveness. This process involves the strategic configuration of the neural network, where each decision reflects an inductive bias—the underlying assumptions embedded in the model through choices in network structure. These biases influence how the model interprets and processes information \citep{battaglia2018relationalinductivebiasesdeep}. 
 The sources of uncertainty pertain to model uncertainty are: 

\textbf{\textit{(1) Model Architecture and Hypothesis Space:}} The architecture of an LLM and the hypothesis space it explores are crucial to its performance and error susceptibility. Architectural decisions, such as the number of layers and network types, significantly influence model effectiveness across various tasks. These choices determine the hypothesis space—what the model can learn and predict—thereby introducing uncertainty in the model’s ability to understand and generate language under different conditions. Variability in architectural setup can cause performance discrepancies when applied to new or varied datasets \citep{fedus2022switchtransformersscalingtrillion, abdar2021review, he2024surveyuncertaintyquantificationmethods, gawlikowski2022survey, dodge2020finetuningpretrainedlanguagemodels}.
% The architecture of an LLM as special type of DNN and the hypothesis space. it explores are critical determinants of its performance and susceptibility to errors. Decisions about the number of layers and types of networks significantly impact the effectiveness of the model across various tasks. Each architectural choice affects the hypothesis space—what the model can learn and predict—introducing uncertainty in how well the model can understand and generate language under different conditions. This variability in the architectural setup can lead to discrepancies in performance when the model is applied to new or varied datasets \citep{,fedus2022switchtransformersscalingtrillion,abdar2021review, he2024surveyuncertaintyquantificationmethods,gawlikowski2022survey, dodge2020finetuningpretrainedlanguagemodels}.


\textbf{\textit{(2) Parameter Estimation and Optimization:}} Parameter estimation and optimization methods are critical sources of variability and uncertainty in LLMs. Choices in optimization techniques (e.g., SGD, Adam), learning rates, loss functions, and regularization methods (e.g., dropout, L2 regularization) significantly impact the model's generalization capabilities and robustness \citep{lakshminarayanan2017simple}. These factors contribute to uncertainty in the model’s ability to consistently replicate results across different runs or datasets, affecting its adaptability to new data and stability across various operational environments \citep{payzan2011risk}.
% The methods and strategies used in parameter estimation and optimization are crucial sources of variability and directly contribute to uncertainty in the performance of Large Language Models (LLMs). Choices in optimization techniques (e.g., SGD, Adam), learning rates, loss functions, and regularization methods (e.g., dropout, L2 regularization) significantly influence the model's generalization capabilities and robustness \citep{lakshminarayanan2017simple}.  This leads to uncertainty in the model’s ability to consistently replicate results across different runs or datasets. These factors introduce a level of uncertainty, as they affect how well the model can adapt to new, unseen data and maintain stability across different operational environments \citep{payzan2011risk}. 









% \end{mdframed}



\subsubsection{Operational Uncertainty in Instruction Tuning and Alignment Stage of LLMs}

Instruction-tuning and Reinforcement Learning from Human Feedback (RLHF) are advanced techniques that enhance LLMs' adaptability and responsiveness to specific tasks or user preferences \citep{ouyang2022training, rafailov2024direct}. These techniques refine model responses to align more closely with expected outcomes using predefined instructions or guidelines \citep{bai2022training, askell2021general}. This process introduces uncertainty through two main sources: 

\textbf{\textit{(1) Inconsistency and Bias in Data Labeling and Human Annotation:}} Human labeling and annotation are fundamental sources of uncertainty in the training LLMs \citep{9022324, Abdar_2021, zhou2024relyingunreliableimpactlanguage}. The subjective nature of human judgment introduces variability and biases, affecting learning outcomes from reward models \citep{zhang-etal-2023-llmaaa}. Individual differences in perception and decision-making can lead to cognitive biases and inconsistency in labeled data, which RLHF reward modeling algorithms may exacerbate \citep{wang2024secretsrlhflargelanguage, denison2024sycophancysubterfugeinvestigatingrewardtampering}.

\textbf{\textit{(2) Interpretation of Guidelines and Feedback:}}The interpretation of instructions can vary, depending on the clarity of the guidelines and the model’s ability to interpret them contextually \cite{wang2024resiliencelargelanguagemodels}. Discrepancies in understanding or applying these instructions can lead to variability in the model’s outputs \citep{siththaranjan2023distributional, wu2024towards, chidambaram2024direct,park2024principled}. The subjective nature of feedback and its interpretation by the model can introduce additional layers of uncertainty. This is particularly evident when there is a lack of consensus among human reviewers, leading to challenges in achieving stable and predictable model behavior \citep{9022324, Abdar_2021, zhou2024relyingunreliableimpactlanguage}.

% Human labeling and annotation are fundamental sources of uncertainty in the training of DNNs and LLMs, particularly during data labeling phases and alignment and Reinforcement Learning from Human Feedback (RLHF) processes \citep{9022324, Abdar_2021, zhou2024relyingunreliableimpactlanguage}. The subjective nature of human judgment can introduce variability and biases into the data, affecting the model's learning outcomes \citep{zhang-etal-2023-llmaaa}. This variability arises from individual differences in perception, interpretation, and decision-making, which may lead to inconsistencies in labeled data. Additionally, RLHF, which adjusts model responses based on human feedback, can further compound this uncertainty, especially when feedback is inconsistent or biased \citep{wang2024secretsrlhflargelanguage}. This variability in human judgment means that the labeled data LLMs learn from may not consistently represent the underlying reality it aims to model. 



% % \begin{mdframed}
% % \textbf{Factor VII\sijia{VI?}: Data Labeling and RLHF as Sources of Uncertainty}\newline
% Human labeling and annotation are fundamental sources of uncertainty in the training of DNNs and LLMs, particularly during data labeling phases and Reinforcement Learning from Human Feedback (RLHF) processes \citep{9022324, Abdar_2021, zhou2024relyingunreliableimpactlanguage}. The subjective nature of human judgment can introduce variability and biases into the data, affecting the model's learning outcomes \citep{zhang-etal-2023-llmaaa}. This variability arises from individual differences in perception, interpretation, and decision-making, which may lead to inconsistencies in labeled data. Additionally, RLHF, which adjusts model responses based on human feedback, can further compound this uncertainty, especially when feedback is inconsistent or biased \citep{wang2024secretsrlhflargelanguage}. This variability in human judgment means that the labeled data LLMs learn from may not consistently represent the underlying reality it aims to model. 
% \end{mdframed}





% \begin{mdframed}
% \textbf{Factor III: Instruction-Tuning and Reinforcement Learning from Human Feedback (RLHF)}\\
% The interpretation of instructions can vary, depending on the clarity of the guidelines and the model’s ability to interpret them contextually \cite{wang2024resiliencelargelanguagemodels}. Discrepancies in understanding or applying these instructions can lead to variability in the model’s outputs. Several works attempt to address such annotator preference heterogeneity\citep{siththaranjan2023distributional, wu2024towards, chidambaram2024direct,park2024principled}. In contrast with traditional reward models predicting the exact reward score, \cite{siththaranjan2023distributional, wu2024towards} train reward models to predict the reward distributions to model the distributional preferences. \cite{chidambaram2024direct,park2024principled} design multiple reward models for crowds with different preferences, then propose aggregation methods to produce a single general reward model. Similarly, RLHF involves adjusting the model's behavior based on feedback from human interactions. While this method is powerful for tailoring model responses to align with human judgments, it inherently incorporates the biases and variability of human feedback into the model. The subjective nature of feedback and its interpretation by the model can introduce additional layers of uncertainty. This is particularly evident when feedback is inconsistent or when there is a lack of consensus among human reviewers, leading to challenges in achieving stable and predictable model behavior \citep{9022324, Abdar_2021, zhou2024relyingunreliableimpactlanguage}. %\sijia{do we need to also discuss other techniques like DPO?}
% % \end{mdframed}


\subsubsection{Operational Uncertainty in Inference Stage of LLMs}

\textbf{\uline{Distributional Uncertainty}} occurs when there are discrepancies between the training data distributions and those encountered during testing, a phenomenon known as dataset shift. This uncertainty is prevalent in real-world applications where models face data significantly different from their training sets. Distributional uncertainty indicates a lack of model familiarity with new data, posing challenges in making accurate predictions. This uncertainty is categorized into in-domain and out-of-domain types.

\textbf{\textit{(1) In-Domain Uncertainty:}} This type of uncertainty occurs when LLMs operate within their training environments and inputs closely resemble the training data distribution. Such scenarios often present interpolation challenges or deal with 'unknown knowns' \citep{ashukha2021pitfallsindomainuncertaintyestimation, H_llermeier_2021}. Despite the similarity to training datasets, subtle nuances and variations within seemingly familiar data can still provoke uncertainties if not fully captured during training \citep{kim2023pseudooutlierexposureoutofdistribution, kong-etal-2020-calibrated}.

\textbf{\textit{(2) Out-of-Domain Uncertainty:}} This occurs when LLMs face queries or data points outside their training distribution, leading to 'unknown knowns' and 'unknown unknowns,' where the model lacks the necessary data or precedent to generate well-founded responses, often resulting in overly generic or shallow outputs \citep{xu2024largelanguagemodelsanomaly, liu2024goodllmsoutofdistributiondetection, kong-etal-2020-calibrated}. 'Unknown knowns' are situations where the model has indirect knowledge but encounters data that, while potentially interpolatable from known data, still lies outside its direct experience, leading to uncertain responses despite possible correctness \citep{amayuelas2023knowledge}. Conversely, 'unknown unknowns' refer to entirely unfamiliar data types or topics that the model has never encountered, typically producing speculative, erroneous, or hallucination.


% Understanding the nuances of in-domain knowledge uncertainties is crucial for comprehending how LLMs function as decision-making agents within the realms of their training environments. These uncertainties primarily arise when inputs closely resemble the data distribution on which the model was trained, encompassing scenarios typically categorized as interpolation challenges or dealing with ``\textbf{\textit{unknown knowns}}'' \citep{ashukha2021pitfallsindomainuncertaintyestimation, H_llermeier_2021}. In-domain uncertainty surfaces even in familiar contexts where the input data aligns well with the training distribution. Despite the apparent familiarity of such data, LLMs can exhibit uncertainties because of subtle nuances and variations within the data that may not be explicitly captured during training \citep{kim2023pseudooutlierexposureoutofdistribution, kong-etal-2020-calibrated}. 


% This occurs when LLMs encounter queries or data points that fall outside their training distribution, leading to 'unknown knowns' and 'unknown unknowns.' Such challenges present significant difficulties as the model lacks the necessary data or precedent to form well-founded responses, resulting in outputs that may be overly generic or lack depth \citep{xu2024largelanguagemodelsanomaly, liu2024goodllmsoutofdistributiondetection, kong-etal-2020-calibrated}. 'Unknown knowns' refer to situations where the model has indirect knowledge but encounters data that could potentially be interpolated from known data, yet it still falls outside its direct experience. This results in responses that might be correct but are not certain due to the lack of direct training \citep{amayuelas2023knowledge}. Conversely, 'known unknowns' involve completely unfamiliar data types or topics that the model has never been trained on, resulting in responses that are speculative at best, and often erroneous or overly generalized. 


\textbf{\uline{Sampling and Decoding Strategy}} is another importatn sources of uncertainty in inference stage originate from the . The configuration of LLMs at inference time, including temperature scaling, context length \citep{anil2022exploringlengthgeneralizationlarge}, and decoding strategies such as beam search or nucleus sampling, significantly affects the uncertainty of model outputs. Temperature scaling adjusts the randomness of predictions by modifying the probability distribution, with lower values resulting in more deterministic outputs and higher values increasing diversity and variability. The choice of context length can influence the extent of uncertainty in outputs, with longer generations potentially introducing more uncertainty than shorter ones. Decoding strategies like beam search enhance output coherence by considering multiple possibilities, yet may reduce variability and creativity. These configurations are crucial for the model’s generalization across tasks, impacting the coherence and consistency of predictions, thus playing a key role in balancing performance with uncertainty \citep{renze2024effectsamplingtemperatureproblem, xie2023selfevaluationguidedbeamsearch, zeng2021improving, ott2018analyzinguncertaintyneuralmachine, hashimoto-etal-2024-beam, stahlberg-byrne-2019-nmt, eikema-aziz-2020-map, meister-etal-2020-beam, fan-etal-2018-hierarchical, Holtzman2020The, hewitt-etal-2022-truncation}.



% \begin{mdframed} \textbf{Factor II: User Uncertainty Uncertainty}\sijia{seems this factor need some more content}\newline
% \begin{itemize}
%     \item Sycophancy
%     \item Ambiguous Input
% In general, ambiguity arise when there exist  disagreement among provided information that can cause due to:

% \textbf{Conflicting Information:} \begin{itemize} \item \textbf{Internal Data Conflicts:} These arise when inconsistencies within the training data, such as contradictory details or labeling inconsistencies, lead to uncertainties in how the model learns and interprets information. Such conflicts can impair the model's ability to form clear and consistent patterns, directly affecting output accuracy. \item \textbf{External Data Conflicts:} Conflicts can also occur when new user inputs clash with the model's pre-trained knowledge. For example, user inputs that contradict the information in the model's training dataset can create significant challenges, forcing the model to navigate discrepancies and potentially leading to uncertain responses. \end{itemize}
% \end{itemize}

% \end{mdframed}

% \subsection{Discussion and Summary of Operational Uncertainty in Large Language Models}

% Data uncertainty in LLMs pertains to the uncertainty that originates directly from the pre-training or input data used during both the training and inference phases. This type of uncertainty is typically due to information loss or inaccuracies in the data representation. For example, in natural language tasks, ambiguity in user queries or textual inputs, such as idiomatic expressions or sarcasm, introduces data uncertainty that LLMs may not be able to resolve. Similarly, errors in data annotation or biased data samples can lead to misinterpretations or unreliable predictions by the model. The complexity of natural language, coupled with the diverse and nuanced ways humans communicate, inherently contributes to this type of uncertainty. On the other hand, model uncertainty in LLMs encapsulates the variability and potential inaccuracies arising from the model's design and training. This includes errors in the training algorithms, inadequate or oversimplified model architectures, or the model's inability to generalize well due to insufficient coverage or diversity in the training dataset. Considering the outlined factors contributing to uncertainties in LLM predictions, model uncertainty typically encompasses issues related to the architecture design, the nuances of training dynamics, and advanced tuning methods such as RLHF. Data uncertainty, on the other hand, is often related to ambiguities and complexities in the textual data itself. 

% While model uncertainties can be theoretically reduced by refining the model architecture, enhancing the training procedures, or diversifying the training data, data uncertainties often present more persistent challenges that cannot be fully eliminated due to the inherent limitations of how data represent complex human language. Thus, developing LLMs capable of handling these uncertainties—by improving their ability to discern and adjust to ambiguities in input data and refining model robustness against varied inputs—is crucial for their successful deployment in mission-critical and safety-critical applications. Such models need to not only identify and manage the intrinsic unpredictability of natural language but also provide reliable and accurate outputs despite these uncertainties.

\subsection{Output Uncertainty in LLMs}
In contrast to operational uncertainties, which stem from the mechanics of how LLMs as deep neural networks generate text, output uncertainties focus on the outputs these models produce when used as knowledge generation tools. This capability can release a vast flow of information useful for decision-making in various downstream tasks. Here, the challenge shifts from a shortage of information to the risks of poorly understanding and managing inherent uncertainties, which may arise from unreliable, incomplete, deceptive, or conflicting information. The topic of reasoning and decision-making under uncertainty has been extensively explored in various AI domains, such as belief/evidence theory and game theory. This extensive knowledge base is crucial for enhancing our understanding of LLM outputs and identifying their inherent uncertainties, important for tasks relying on this knowledge. Building on insights from a recent survey on uncertainty and belief theory \citep{guo2022surveyuncertaintyreasoningquantification}, we adapted their framework to classify uncertainties better suited to the characteristics of LLM outputs. As a result, we categorize the sources and causes of output uncertainties based on the \textbf{\textit{ambiguity}} in the output itself, which can stem from various causes and sources as: 

\textbf{\textit{(1) Lack of supporting evidences and incomplete knowledge:}} An LLM may produce outputs with uncertainties due to a lack of supporting evidence in the responses, a common occurrence even in well-trained models addressing complex or nuanced topics. This uncertainty stems from the model generating conclusions without sufficient evidence to substantiate its answers, and from its inability to provide sufficient theoretical understanding or reliable information. The connections between claims and supporting information may not be clearly established or detailed, which hampers confident and reliable reasoning and decision-making. To mitigate this, the model's output can be enriched by incorporating more robust evidence or discarding unreliable evidence. Additionally, the complexity of model-generated information can overwhelm users due to limited cognitive capacity to process dense or intricate data. Simplifying the data into more manageable chunks with coarser granularity or focusing on key features while omitting less critical details can help. Effectively managing this uncertainty involves concentrating on leveraging the most relevant information available, thus enhancing the confidence and trust in the accuracy and relevance of the outputs. 

\textbf{\textit{(2) Multiple knowledge frames and contradicting knowledge :}} These sources of uncertainty arise in scenarios where the same information—such as evidence or opinions—can be interpreted in various ways, leading to conflicting views. Multiple, valid beliefs about certain knowledge or information may coexist, often due to conflicting evidence. Conflicts can occur when parts of the information are incorrect, irrelevant, or when the model interpreting the data is not suitable for the current context. Additionally, conflicts may arise where there is no definitive ground truth, or in cases of controversial debate. Differing opinions from users, based on subjective perspectives, further complicate understanding and increase the layers of uncertainty.



% This refers to scenarios where insufficient knowledge or evidence impedes confident and reliable reasoning and decision-making. This form of uncertainty may stem from a dearth of evidence or from the model's inability to provide sufficient theoretical understanding or reliable information. Mitigating this uncertainty involves enriching the model's output with more robust evidence or by discarding unreliable evidence. Additionally, complexity in the model-generated information can overwhelm users due to their limited cognitive capacity to process dense or intricate data. One way to address this  is by simplifying the data into more manageable chunks with a coarser granularity or by emphasizing key features while omitting less critical details. Effectively managing this uncertainty requires focusing on and leveraging the most relevant information from what is available. 

% In general, ambiguity arise when there exist  disagreement among provided information that can cause due to:

% \textbf{Conflicting Information:} \begin{itemize} \item \textbf{Internal Data Conflicts:} These arise when inconsistencies within the training data, such as contradictory details or labeling inconsistencies, lead to uncertainties in how the model learns and interprets information. Such conflicts can impair the model's ability to form clear and consistent patterns, directly affecting output accuracy. \item \textbf{External Data Conflicts:} Conflicts can also occur when new user inputs clash with the model's pre-trained knowledge. For example, user inputs that contradict the information in the model's training dataset can create significant challenges, forcing the model to navigate discrepancies and potentially leading to uncertain responses. \end{itemize}

% \subsubsection{In-Domain Uncertainty}


% Understanding the nuances of in-domain knowledge uncertainties is crucial for comprehending how LLMs function as decision-making agents within the realms of their training environments. These uncertainties primarily arise when inputs closely resemble the data distribution on which the model was trained, encompassing scenarios typically categorized as interpolation challenges or dealing with ``\textbf{\textit{unknown knowns}}'' \citep{ashukha2021pitfallsindomainuncertaintyestimation, H_llermeier_2021, }\sijia{either miss a reference or there's an extra comma}. In-domain uncertainty surfaces even in familiar contexts where the input data aligns well with the training distribution. Despite the apparent familiarity of such data, LLMs can exhibit uncertainties because of subtle nuances and variations within the data that may not be explicitly captured during training \citep{kim2023pseudooutlierexposureoutofdistribution, kong-etal-2020-calibrated}.





% \textbf{Incomplete Knowledge:} 
% \begin{itemize}
% \item \textbf{Out-of-Domain Uncertainty:} This occurs when LLMs encounter queries or data points that fall outside their training distribution, leading to ``unknown knowns'' and ``unknown unknowns.'' Such challenges present significant difficulties as the model lacks the necessary data or precedent to form well-founded responses, resulting in outputs that may be overly generic or lack depth \citep{xu2024largelanguagemodelsanomaly, liu2024goodllmsoutofdistributiondetection, kong-etal-2020-calibrated}. 

% \begin{itemize} \item \textbf{Unknown Knowns:} These are situations where the model has indirect knowledge but
% encounters data that could potentially be interpolated from known data, yet it still falls
% outside its direct experience. This results in responses that might be correct but are
% not certain due to the lack of direct training \citep{amayuelas2023knowledge}. \sijia{what is the difference between in-domain unknown knowns and out-of-domain unknown knowns?}
% \item \textbf{Known Unknowns:} These scenarios involve completely unfamiliar data types or topics that the model has never been trained on, resulting in responses that are speculative at best, and often erroneous or overly generalized \citep{amayuelas2023knowledge}.
% \end{itemize} 

% \paragraph{Lack of Supporting Evidence:} Even within its domain, an LLM may produce responses based on insufficient or sparse evidence from the training data. This is particularly evident when the data lacks the necessary depth or breadth to cover complex or niche topics adequately. \sijia{remove extra end\{itemize\}}


% \subsubsection{Incomplete Knowledge and Conflicting Information}

% In the realm of Large Language Models (LLMs), which operate as advanced decision-making agents, handling uncertainties arising from incomplete knowledge and conflicting information is pivotal. These uncertainties not only challenge the model's effectiveness but also affect its reliability in critical decision-making scenarios.

% \paragraph{Incomplete Knowledge:} Incomplete knowledge refers to the model's limitations in understanding or accessing complete information. This often manifests in two primary forms:

% \begin{itemize} \item \textbf{Out-of-Domain Uncertainty:} This occurs when LLMs are presented with queries or scenarios that fall outside their training distribution, termed as "unknown knowns" and "unknown unknowns." Such inputs pose significant challenges due to the model's lack of direct experience or adequate data representation. \begin{itemize} \item \textbf{Unknown Knowns:} These are scenarios where the model has some relevant, albeit indirect, knowledge that could be interpolated from its existing data but is not explicitly covered. \item \textbf{Unknown Unknowns:} These involve completely new or unfamiliar topics and data types, for which the model has no prior training or conceptual framework. \end{itemize} \item \textbf{Lack of Supporting Evidence:} This issue emerges even within familiar domains, where the LLM must generate responses or make decisions based on insufficient or vague data from its training set. This often leads to speculative or overly generalized outputs. \end{itemize}

% \paragraph{Conflicting Information:} LLMs also face uncertainties due to conflicting information, which can arise internally from the training data or externally from user inputs:

% \begin{itemize} \item \textbf{Internal Data Conflicts:} These occur when the training data itself contains contradictory information or inconsistent labeling, which complicates the model's learning process and leads to ambiguous outputs. \item \textbf{External Data Conflicts:} When new inputs from users clash with the pre-trained knowledge of the model, it must navigate these discrepancies. Such conflicts challenge the LLM's operational integrity and can lead to unpredictable responses. \end{itemize}

% \subsection{Discussion on Methods to Estimate the Output Uncertainty}

% \Mo{There are some methods that try to quantify the above uncertainties in "other" domains. However, there is no work based on these methods on LLM literature. I am wondering should I discuss them here or in main discussion/future direction section of the paper?}




==> ICLR_2025_Template/Sections/5.methods.tex <==
 \section{Approaches for Estimating and Evaluating Uncertainty in LLMs}
\label{sec: methods}

Existing approaches to assess how well a model understands and is certain about its predictions in LLMs can be summarized into four major categories: 
%literature can be categorized into four major approaches: %logit-based, self-evaluation, consistency-based, and internal-based.

\textbf{Logit-based} approaches \citep{Lin2022TeachingMT, mielke-etal-2022-reducing, jiang-etal-2021-know, kuhn2023semantic} assess model confidence by analyzing the probability distributions or entropy of outputs, providing clear measures of confidence. Although straightforward to implement, a fundamental issue with using logits as confidence indicators is that they reflect the probability distribution across potential tokens (vocabulary space), capturing linguistic forms rather than verifying the truthfulness or correctness of statements \citep{Lin2022TeachingMT, si2022reexamining, tian2023just}. Logit probabilities, irrespective of their magnitude, predominantly represent distribution over vocabulary space. Therefore, logit probabilities do not directly indicate model uncertainty but also reveal various linguistic factors that influence the model’s output. This nuanced perspective is in stark contrast to human expressions of certainty, which typically reflect a belief in the accuracy or truth of a claim, based on information processing and decision-making processes, and are not influenced by phrasing \citep{koriat1980reasons, fischhoff1977knowing}. Additionally, another significant limitation is that logit-based methods do not identify or measure any types of uncertainty, limiting their applicability in scenarios where understanding the sources and degrees of uncertainty is crucial.

\textbf{Consistency-based} approaches \citep{vazhentsev-etal-2023-efficient, portillo-wightman-etal-2023-strength, wang2023selfconsistency, shi2022natural, manakul2023selfcheckgpt, agrawal2023language} assess confidence by evaluating the agreement among various model responses, identifying potential inconsistencies. However, these methods encounter significant challenges, especially due to the diversity of potential paraphrases and formatting variations in textual data, complicating their use in real-time scenarios \citep{xiong2024llms, jiang-etal-2021-know, fadaee-etal-2017-data, Li_2022, ding2024data, kuhn2023semantic}. Additionally, a non-trivial challenge is the effective measurement of consistency among responses, a persisting issue that hinders accurate confidence assessment \citep{manakul2023selfcheckgpt, zhang2023siren}.

\textbf{Self-evaluation} methods \citep{kadavath2022language, manakul2023selfcheckgpt, lin2024generating} enable models to internally assess the correctness of their answers by leveraging their introspective capabilities. These methods employ various prompts that encourage models to express their confidence through numerical values or verbalized terms. Recent studies have refined these approaches, utilizing strategies like Chain of Thought (CoT) to enhance how models calibrate and articulate linguistic confidence \citep{xiong2023can}. Research has also explored expressing confidence with linguistics qualifiers to better align verbal expressions with the model’s actual confidence levels \citep{mielke2022reducing, zhou2023navigating, lin2022teaching}, making model outputs more understandable for users. Despite their potential, these methods are constrained by the model’s limited self-awareness, which can lead to circular reasoning and overconfident inaccuracies \citep{ji-etal-2023-towards, chen-etal-2023-adaptation}. Another challenge is the interpretability and validity of obtained probabilities that align with specific linguistic and psychological interpretations, including expressions like 'I think,' 'undoubtedly,' or 'high confidence.'

\textbf{Internal-Based Approach} Recently, \citet{beigi2024internalinspectori2robustconfidence} used a mutual information framework to theoretically demonstrate that the internal states of large language models provide additional insights into the correctness of their answers. \citet{burns2023discovering} introduced an innovative unsupervised method that maps hidden states to probabilities. This approach involves responding to "Yes" or "No" questions, extracting model activations, converting these activations into probabilities. Furthering this research, studies have employed linear probes \citep{li2023inference, azaria2023internal} and contrastive learning \citep{beigi2024internalinspectori2robustconfidence} to assess whether the internal states across various layers can distinguish between correct and incorrect answers. Empirical results suggest that certain middle layers and specific attention heads show strong discriminative abilities. \citet{beigi2024internalinspectori2robustconfidence} expanded these findings by illustrating that for tasks requiring contextual processing, such as reading comprehension, the outputs of multi-head self-attention (MHSA) components are crucial for assessing response correctness. However, current methodologies exhibit limitations. Each task and dataset requires training a specific ``confidence estimator'' model, which restricts their generalizability. This limitation is evident as the performance of these methods often declines when trained on one task and dataset and tested on another, highlighting their limited transferability across different applications \citep{bashkansky2023surely}. Additionally, the computational resources required to train these confidence estimators pose challenges for their deployment in real-time applications, further complicating their practical utility.

\textbf{What are the main properties of these methods in estimating uncertainty in LLMs?} Table \ref{tab: compare} outlines the key characteristics of the methods discussed in this study, including their complexity, computational effort, memory consumption, flexibility, and their ability to identify and measure sources of uncertainty in LLMs.

\input{ICLR_2025_Template/Tables/methods}






==> ICLR_2025_Template/Sections/6.discussion.tex <==
\textbf{Go beyond Confidence Estimation:} As discussed, the literature on uncertainty estimation in LLMs primarily interprets confidence scores as measures of uncertainty. Such a prevalent method oversimplifies the nuanced and complex nature of uncertainty inherent in model predictions, which is crucial for accurate interpretation and reliability of model outputs. The limitations inherent in current methodologies necessitate the development of a more advanced framework for categorizing uncertainty estimation in large language models that surpasses the reliance on simple confidence scores. 

\textbf{Lack of Explainability:} Current methods of confidence estimation provide certainty predictions without elucidating the underlying causes of potential uncertainties. While these scores may seem reasonable to human observers, the absence of insight into the sources of uncertainty complicates trust in the model's outputs, particularly in safety-critical contexts where explainability is essential. Current confidence quantification techniques struggle to pinpoint specific weaknesses or improvement areas in the model. Additionally, these methods lack the necessary transparency to clarify the reasons for model uncertainty, whether due to input ambiguity from users, insufficient knowledge, or conflicting information in the training data.

\textbf{Lack of Ground Truth for Uncertainty Estimation:} Current methods for estimating uncertainty are empirically evaluated and assess how accurately they predict the correctness of an answer. However, there is generally no established ground truth for validation, particularly regarding the sources of uncertainty, meaning currently there is no metric and method to determine the contribution of different uncertainties for specific models and tasks.

\textbf{Lack of Transferability of Uncertainty Estimation Methods Across Different Applications and Datasets:} Current uncertainty estimation methods often struggle with adaptability and generalizability when applied to new applications or datasets. Although effective within their specific domains, these methods frequently fail to yield reliable results in different settings due to factors like data distribution differences and unique domain-specific requirements. To overcome these limitations, it is crucial to develop more robust and flexible uncertainty estimation techniques that can adjust to the varied conditions and demands of diverse applications.

\textbf{Lack of Standardized Evaluation Protocol \& Comprehensive Benchmarks for Confidence Estimation:} Current methods for evaluating uncertainty estimation methods are typically used to compare uncertainty quantification techniques through metrics like accuracy, calibration, or performance in out-of-distribution detection, using standardized datasets common within the LLM community. Despite this, variations in experimental settings across studies highlight the need for a comprehensive benchmark across tasks and domains to assess their robustness. The absence of a standardized testing protocol poses challenges for researchers from different downstream tasks, making it difficult to identify the most advanced methods or choose a specific sub-field of uncertainty quantification to pursue. This lack of uniformity hinders the direct comparison of emerging techniques and impedes the broader acceptance and integration of established uncertainty quantification methods.








% Existing methods for evaluating estimated uncertainty, primarily used to compare uncertainty quantification methods through calibration or performance on out-of-distribution detection, employ standardized datasets within the LLM community. However, confidence estimation and calibration are widely applicable, and a comprehensive benchmark across tasks and domains is crucial to evaluate their robustness and utility effectively. This is particularly important given the extensive human effort required to annotate LLM responses, especially in long-form generation contexts. Segmenting long outputs of LLMs for these assessments, rather than treating them as a whole, can significantly improve their precision and effectiveness. Despite this, experimental settings vary across studies and there is no standardized protocol for testing, making it challenging for researchers from other fields to identify state-of-the-art methods or decide which sub-field of uncertainty quantification to focus on. This lack of standardization complicates the direct comparison of new approaches and hampers the acceptance and adoption of existing uncertainty quantification methods.
% Existing methods for evaluating estimated uncertainty are primarily used to compare uncertainty quantification methods through measurable quantities like calibration or performance on out-of-distribution detection, using standardized datasets within the LLM community. However, the experimental settings can vary across studies, and there is no standardized protocol for testing these methods. This lack of standardization makes it challenging for researchers from other fields to identify state-of-the-art methods or decide which sub-field of uncertainty quantification to focus on. Consequently, this complicates the direct comparison of new approaches and hampers the acceptance and adoption of existing uncertainty quantification methods.





% \paragraph{Go beyound Confidence Estimation}

% The limitations inherent in current methodologies necessitate the development of a more advanced framework for categorizing uncertainty estimation in large language models that surpasses the reliance on simple confidence scores. This proposed framework should embrace the unique characteristics of text as a data type and acknowledge the critical role of LLMs as knowledge providers for decision-making in downstream tasks. It must thoroughly identify and categorize the sources, mechanics, and dynamics through which uncertainty enters the model across various phases of its lifecycle: from pre-training and fine-tuning to inference and output interpretation.


% \paragraph{Mitigating Uncertainty by Understanding Sources in the Development Process}

% An integral part of enhancing the performance and trustworthiness of LLMs involves understanding and mitigating the sources of uncertainty during their development process. This initiative requires a deep dive into the inception, evolution, and operational phases of LLMs, examining how each phase contributes to the accumulation of uncertainty. From the initial data collection and model training to fine-tuning and real-world deployment, each step offers unique challenges and opportunities for introducing or addressing uncertainties.

% For instance, during the pre-training phase, uncertainties might stem from the diversity and representativeness of the training data or from the architectural choices made. During fine-tuning, the model's adaptability to specific tasks can introduce or reveal new uncertainties, particularly related to overfitting or underfitting to niche datasets. In the deployment phase, the way an LLM interacts with end-user inputs and how it handles unexpected or out-of-distribution data can significantly affect its performance reliability.

% \paragraph{Calibration to Human Variation}

% Human variation significantly complicates the calibration of LLMs. As highlighted by recent studies, humans often have different opinions when labeling the same data due to task ambiguity, annotator subjectivity, and input ambiguity. This misalignment between LLM calibration measures and human disagreement underscores the need for models that can handle various types of ambiguity effectively. Measures such as abstaining from answering ambiguous questions and resolving ambiguity are crucial for developing trustworthy and reliable LLMs that are well-aligned with human variation.


